Is an Object-Centric Video Representation Beneficial for Transfer?

The objective of this work is to learn an object-centric video representation, with the aim of improving transferability to novel tasks, i.e., tasks different from the pre-training task of action classification. To this end, we introduce a new object-centric video recognition model based on a transformer architecture. The model learns a set of object-centric summary vectors for the video, and uses these vectors to fuse the visual and spatio-temporal trajectory 'modalities' of the video clip. We also introduce a novel trajectory contrast loss to further enhance objectness in these summary vectors. With experiments on four datasets -- SomethingSomething-V2, SomethingElse, Action Genome and EpicKitchens -- we show that the object-centric model outperforms prior video representations (both object-agnostic and object-aware), when: (1) classifying actions on unseen objects and unseen environments; (2) low-shot learning of novel classes; (3) linear probe to other downstream tasks; as well as (4) for standard action classification.

==> sections/ablation.tex <==
\section{Ablation}


==> supp_sections/aux.tex <==
\section{Other auxiliary losses}
We have tried applying some other types of auxiliary losses on the object summary output from our Object Learner. 
Results (\Cref{tab:auxloss}) show that they do not help achieve a better performance on downstream tasks, hence are not included in the main paper. 
We list them below as supplementary materials.
% Here we listed different types of losses we have explored and their performance on action recognition and hand contact state detection.
% According to our experiment results, they do not help achieve better results on downstream tasks than having single instance-level contrastive loss on object trajectories.
\subsection{Instance-level contrastive loss on visual affinity vectors}
Given the visual feature maps of a clip and the bounding boxes of an object in it, 
we ROI-Pool the object features $w_j$ from each frame, where j is the index of object. Using these per-frame object features, we compute the transformation vectors between frames:

\begin{equation}
    \mathbf{\tilde{aff}}^i_j =
    \mathbf{w}^i_j \cdot \mathbf{\transpose{w}}^{i+1}_j ,
\end{equation}
We embed the transformation vectors of an object along the temporal dimension into one feature vector $z_j$ and its shuffled version $z^{shuffle}_j$. The encoding is done by using a small Transformer $g(.)$ with 2 layers and 4 heads.
\begin{equation}
    \mathbf{z_j} = g(\mathbf{\tilde{aff}}_j),
\end{equation}
\begin{equation}
    \mathbf{z}^{shuffle}_j = g(\mathbf{\tilde{aff}}^{shuffle}_j),
\end{equation}
\begin{equation}
\mathbf{\tilde{aff}}_j= (\mathbf{\tilde{aff}}^1_j, \mathbf{\tilde{aff}}^2_j, \hdots,\mathbf{\tilde{aff}}^{T'-1}_{j})
\end{equation}
\begin{equation}
    \mathbf{\tilde{aff}}^{shuffle}_j= Shuffle(\mathbf{\tilde{aff}}^1_j, \mathbf{\tilde{aff}}^2_j, \hdots,\mathbf{\tilde{aff}}^{T'-1}_{j})
\end{equation}
$z_j$ and $z^{shuffle}_j$ are used in the contrastive loss against object summary vectors $s_j$ as in:
\begin{equation}
    \mathcal{L}_{aff}=-\sum_{j}\Bigg[\log{\frac{ \exp(\transpose{s}_{j} \cdot {z}_{j} ) }
        {\sum_{k}{\exp(\transpose{s}_{j} \cdot {z}_{k})}+ \sum_{k}{\exp(\transpose{s}_{j} \cdot {z}^{shuffle}_{k})} } }\Bigg] 
    \label{eq:aux-aff}
\end{equation}
    


\subsection{Class-level contrastive loss on ROI-Pooled object vectors}
For each object $j$, we know the action class label $l$ it is associated with. 
We apply a supervised contrastive loss on each object summary vector $s_j$,
where other vectors with the same class label $l$ are treated as its positive samples, with different class labels are treated as negative samples.

\begin{equation}
    \mathcal{L}_{obj}=-\sum_{j}\Bigg[\log{\frac{\sum_{k}\exp(\transpose{s}_{j,l} \cdot {s}_{k,l} ) }
        {\sum_{k}\exp(\transpose{s}_{j,l} \cdot {s}_{k,l}) + \sum_{m,l'\neq l}{\exp(\transpose{s}_{j,l} \cdot {s}_{m,l'})} } }\Bigg] 
    \label{eq:aux-obj}
\end{equation}

\begin{table}[]
    \centering
    \resizebox{0.6\textwidth}{!}{%
    \begin{tabular}{c|c|c|l}
    \textbf{Loss}                   & \textbf{OL only} & \textbf{Backbone only} & \textbf{Final} \\ \hline
    $L_{traj}$                     &   71.0      &    72.0           &   73.6    \\
    $L_{traj} + L_{aff}$           &  71.0       &   72.1            &    73.5   \\
    $L_{traj} + L_{aff} + L_{obj}$ &  70.0       &    72.2           &    73.2   \\ \hline
    \end{tabular}%
    }
    \vspace{2mm}
    \caption{\textbf{Ablation on different types of auxiliary losses on SomethingElse.} Adding other auxiliary losses do not improve the action classification results. We choose to use a single contrastive loss on trajectories (Eq.1 in main paper) for simplicity.}
    \label{tab:auxloss}
    \end{table}

==> tables/scene_graph.tex <==
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.5}
\begin{wraptable}[]{}{6cm}
    \vspace{-5mm}
    \centering
    \resizebox{0.5\textwidth}{!}{%
    \begin{tabular}{cccccc}
    \hline
    \textbf{Method}& \textbf{Boxes} & \textbf{Aux Loss} & \textbf{R@10} & \textbf{R@20} \\ \hline
    MF        & N           & N                  & 76.4                   &   82.6                 \\
    MF+STLT(LCF)    & Y               & N                  & 78.3                   &   83.5                 \\ \hline
    MF+STLT+OL(ours) & Y   & N                  & 78.9                  &    83.8                \\
    MF+STLT+OL(ours)  & Y  & Y                  & \textbf{80.9}                   &  \textbf{85.4}                 \\ \hline
    \end{tabular}%
    }
    \caption{\textbf{Scene graph predicate prediction on Action Genome.} We freeze the model trained on action classification, and linear probe on the output vector to predict predicate between human and object. }
    \label{tab:scene-graph}
    \vspace{-5mm}

 \end{wraptable}

==> tables/visual_input.tex <==
\begin{wraptable}[]{}{6cm}
    \renewcommand{\arraystretch}{1.3}
    \setlength{\tabcolsep}{6pt}
    \resizebox{0.5\textwidth}{!}{%
    \begin{tabular}{cccc}
    \hline
    \textbf{\begin{tabular}[c]{@{}c@{}} Input \\ Visual layer \end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Obj Learner \\ Top1\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Backbone \\ Top1\end{tabular}}& \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}} Averaged \\ Top1\end{tabular}}} \\ \hline
    6                                                                                       & 71.0                                                                   &             72.0                  & \textbf{73.6}                                            \\
    8                                                                                    & \textbf{71.3}                                                                      &             \textbf{72.3}                  & 73.1                                        \\ 
    12                                                                                    & 70.9                                                                     &              72.1                 & 72.0                                           \\\hline
    \end{tabular}%
    }
    \caption{\textbf{Ablations on the Visual Input in Object Learner.} We evaluate the performance of our model with the Object Learner extracting features from layer 6,8,12 in the visual backbone of depth 12. Results show reading from the sixth layer yield best performance.}
    \label{tab:visual-layers}
    \vspace{-6mm}
    \end{wraptable}

